Singularity Structure of N=2 Supersymmetric Yang-Mills Theories: A Review

In this review, we consider the case where electrons, magnetic monopoles, and dyons become massless. Here we consider the ${\cal N} = 2$ supersymmetric Yang-Mills (SYM) theories with classical gauge groups with a rank r, SU(r+1), SO(2r), Sp(2r), and SO(2r+1). which are studied by Riemann surfaces called Seiberg-Witten curves. We discuss physical singularity associated with massless particles, which can be studied by geometric singularity of vanishing 1-cycles in Riemann surfaces in hyperelliptic form. We pay particular attention to the cases where mutually non-local states become massless (Argyres-Douglas theories), which corresponds to Riemann surfaces degenerating into cusps. We discuss non-trivial topology on the moduli space of the theory, which is reflected as monodromy associated to vanishing 1-cycles. We observe how dyon charges get changed as we move around and through singularity in moduli space.

==> 00README <==
<?xml version="1.0" encoding="UTF-8"?>
<!DOCTYPE html PUBLIC "-//W3C//DTD XHTML 1.0 Transitional//EN" "http://www.w3.org/TR/xhtml1/DTD/xhtml1-transitional.dtd">
<html xmlns="http://www.w3.org/1999/xhtml" lang="en">
<head>
<title>arXiv.org help - The 00README.XXX file</title>
<link rel="shortcut icon" href="/favicon.ico" type="image/x-icon" />
<link rel="stylesheet" type="text/css" media="screen" href="/css/arXiv.css" />
<base href="http://arxiv.org/help/00README" />
</head>
<body class="with-cu-identity">
<div id="cu-identity">
<div id="cu-logo">
<a id="insignia-link" href="http://www.cornell.edu/"><img src="/icons/cu/cul_signature_unstyled.gif" alt="Cornell University" width="283" height="76" border="0" /></a>
<div id="unit-signature-links">
<a id="cornell-link" href="http://www.cornell.edu/">Cornell University</a>
<a id="unit-link" href="http://www.library.cornell.edu/">Library</a>
</div>
</div>
<div id="support-ack">
<a href="https://confluence.cornell.edu/x/9YhjCg">We gratefully acknowledge support from<br />the Simons Foundation<br /> and member institutions</a>
</div>
</div>
<div id="header">
<h1><a href="/">arXiv.org</a> &gt; <a href="/help">help</a></h1>
<form id="search" method="post" action="/search">
<div class="search-for">Search or Article-id</div>
<div class="links">(<a href="/help">Help</a> | <a href="/find">Advanced search</a>)</div>
<input type="text" name="query" size="24" maxlength="64" />
&nbsp;
<select name="searchtype">
<option value="all" selected="selected">All papers</option>
<option value="ti">Titles</option>
<option value="au">Authors</option>
<option value="abs">Abstracts</option>
<option value="ft">Full text</option>
<option value="help">Help pages</option>
</select>
<input type="submit" value="Go!" /><br />
</form>
</div>
<div id="content">
<form method="get" action="/help/search">
<a href="/help/">Help Table of Contents</a> &nbsp;|&nbsp;
<input type="hidden" name="method" value="and" />
<input type="hidden" name="format" value="builtin-short" />
<input type="hidden" name="sort" value="score" />
<input type="text" name="words" size="24" maxlength="200" />
<input type="submit" value="Search arXiv Help" />
</form>
<h1>The 00README.XXX file</h1>

<p>
A file of this name can used to specify special handling for the submission and/or for individual files.
The name of the file is spelled &quot;zero-zero-README-dot-X-X-X&quot;.
</p>
<p>
The <code>00README.XXX</code> file is read line-by-line before files are processed by 
AutoTeX. The order of lines is unimportant.
</p>
<ul>
  <li>
    <a href="#ignoring">Ignoring files within the submission package</a>
  </li>
  <li>
    <a href="#including">Including files normally ignored</a>
  </li>
  <li>
    <a href="#toplevel">Declaring your top-level LaTeX file</a>
  </li>
  <li>
    <a href="#landscape">Enabling Landscape mode in <code>dvips</code> submissions only</a>
  </li>
  <li>
    <a href="#nohypertex">Disabling HyperTeX for your submission</a>
  </li>
  <li>
    <a href="#keepcomments">Keep comments within figures during <code>dvips</code></a>
  </li>
  <li>
    <a href="#nostamp">Turn off the arXiv stamp on the generated PostScript and PDF files</a>
  </li>
  <li>
    <a href="#fontmap">Defining a custom fontmap file</a>
  </li>
</ul>

<a name="ignoring" id="ignoring"></a>
<h2>Ignoring files</h2>
<p>
Include lines such as:
</p>

<pre>
filename1.ext1 ignore
filename2.ext2 ignore
</pre>
<p> 
This is useful if you have included other files which are not necessary for
processing and don't belong into a subdirectory for ancillary material either.
</p>

<a name="including" id="including"></a>
<h2>Including files -- not ignoring and not reporting junk</h2>
<p>
Include lines such as:
</p>

<pre>
filename1.whatever include
filename2.whatever include
</pre>

<p>
This will stop detection of unknown file type and will thus stop
the file being given to AutoTeX. This can be used to
include extra files linked from an HTML submission.
</p>

<a name="toplevel" id="toplevel"></a>
<h2>Declaring the top-level (parent) TeX file</h2>
<p>
It is very rarely necessary to do this explicitly because arXiv employs a series
of heuristics which can usually determine the top-level file. 
For example, if only one of a set of LaTeX files contains a
<code>\documentclass</code> command, that file is very likely the top-level 
file.
</p>
<p> 
If it is necessary, however, include a line that says:
</p>

<pre>
myMainTexFile.tex toplevelfile
</pre>

<p> 
where <code>myMainTexFile.tex</code> is the name of the parent TeX file.
</p>

<a name="landscape" id="landscape"></a>
<h2>Landscape mode</h2>
<p>
It is possible to tell AutoTeX to send a flag to <code>dvips</code> requesting 
landscape mode. This sometimes results in upside-down output,
but there is currently no facility to fix this. The command is:
</p> 

<pre>
filename.dvi landscape
</pre>

<p> 
where <code>filename.dvi</code> is the name of the DVI file that TeX will
produce when processing the submission, and <code>filename</code> is the main 
TeX file without the <code>.tex</code> extension. Also, we have an extensive help
library on setting the 
<a href="faq/landscape" title="arXiv landscape help page">landscape environment</a>.
</p>

<a name="nohypertex" id="nohypertex"></a>
<h2>Disable attempt to use HyperTeX</h2>
<p>See also: <a href="faq/mistakes#nohypertex">Disabling hypertex</a>.</p>

<pre>
nohypertex
</pre>

<p>
This stops any attempt by arXiv to automatically augment a paper with
hyperlinks.  However, it does not affect any facilities explicitly used within the
paper's source.  There is no filename associated with this switch.
</p>

<a name="keepcomments" id="keepcomments"></a>
<h2>Keep comments when doing <code>dvips</code></h2>
<p>This is mostly needed when receiving a 
<a href="faq/mistakes#psbad"><code>PS BAD</code> warning</a> 
</p>

<pre>
filename.dvi keepcomments
</pre>

<p> 
Sends the <code>-K0</code> flag to <code>dvips</code>, telling it not to strip comments. This
is needed when PS/EPS figures (included in the DVI) contain 
binary data having '<code>%</code>' characters at the beginning of lines 
(by default, our <code>dvips</code> processor interprets these lines as comments),
 or if the comments are required for some other reason (e.g., Adobe Illustrator output).
</p> 
<p>
Note that <code>filename.dvi</code> is the name of the DVI file that TeX will
produce when processing the submission, and <code>filename</code> is the main 
TeX file without the <code>.tex</code> extension.
</p>
<p>
Also note that it may be necessary to rename your <code>.TEX</code>
files to <code>.tex</code> for this function to work properly.
</p>

<a name="nostamp" id="nostamp"></a>
<h2>Stopping the addition of the arXiv stamp</h2>

<pre>
nostamp
</pre>

<p> 
This tells AutoTeX not to add the arXiv stamp to the 
left-hand edge of the page. No filename is specified.
</p> 

<a name="fontmap" id="fontmap"></a>
<h2>Defining a custom font mapping</h2>

<p>
You can bundle non-standard or custom fonts with your submission and
instruct <code>dvips</code> to use an additional font map file, e.g. <code>myfonts.map</code>,
so that <code>dvips</code> is executed with the fontmap option:
</p>

<code>dvips -u+./myfonts.map</code>

<p>
by adding a file called 00README.XXX to your  submission with the directive:
</p>

<pre>
myfonts.map fontmap
</pre>

<p>
which identifies your private font map file as a <code>dvips</code> fontmap. For
map file syntax consult the dvips info pages. Many font bundles from
<a href="http://www.ctan.org/">CTAN</a> come with their custom font map files, 
and you can use these as is with this directive.

The file name of the font map file must have extension &quot;<code>.map</code>&quot; 
and it must consist of letters <code>A-Z, a-z</code> only.
</p>
</div>
<div id="footer">
<address>
<a href="/help/contact">Contact</a>
</address>
</div>
</body>
</html>

